Combinatorics of the 2-species exclusion processes, marked Laguerre histories, and partially signed permutations

Starting from the two-species partially asymmetric simple exclusion process, we study a subclass of signed permutations, the partially signed permutations, using the combinatorics of Laguerre histories. From this physical and bijective point of view, we obtain a natural descent statistic on partially signed permutations; as well as partially signed permutations patterns.

==> figures/stateAAD.tex <==
\begin{tikzpicture}
  \node[draw,circle,fill=gray!50] (3) at (0,0) {};
  \node[draw,circle,fill=gray!50] (4) at (0.43,0) {};
  \node[draw,circle,fill=black] (5) at (0.86,0) {};
\end{tikzpicture}


==> figures/stateAAE.tex <==
\begin{tikzpicture}
  \node[draw,circle] (3) at (0.86,0) {};
  \node[draw,circle,fill=gray!50] (4) at (0.43,0) {};
  \node[draw,circle,fill=gray!50] (5) at (0,0) {};
\end{tikzpicture}


==> figures/stateADA.tex <==
\begin{tikzpicture}
  \node[draw,circle,fill=gray!50] (3) at (0,0) {};
  \node[draw,circle,fill=black] (4) at (0.43,0) {};
  \node[draw,circle,fill=gray!50] (5) at (0.86,0) {};
\end{tikzpicture}


==> figures/stateAEA.tex <==
\begin{tikzpicture}
  \node[draw,circle] (3) at (0.43,0) {};
  \node[draw,circle,fill=gray!50] (4) at (0,0) {};
  \node[draw,circle,fill=gray!50] (5) at (0.86,0) {};
\end{tikzpicture}


==> figures/stateDAA.tex <==
\begin{tikzpicture}
  \node[draw,circle,fill=black] (3) at (0,0) {};
  \node[draw,circle,fill=gray!50] (4) at (0.43,0) {};
  \node[draw,circle,fill=gray!50] (5) at (0.86,0) {};
\end{tikzpicture}


==> figures/stateEAA.tex <==
\begin{tikzpicture}
  \node[draw,circle] (3) at (0,0) {};
  \node[draw,circle,fill=gray!50] (4) at (0.43,0) {};
  \node[draw,circle,fill=gray!50] (5) at (0.86,0) {};
\end{tikzpicture}

